CSRec: Rethinking Sequential Recommendation from A Causal Perspective

The essence of sequential recommender systems (RecSys) lies in understanding how users make decisions. Most existing approaches frame the task as sequential prediction based on users' historical purchase records. While effective in capturing users' natural preferences, this formulation falls short in accurately modeling actual recommendation scenarios, particularly in accounting for how unsuccessful recommendations influence future purchases. Furthermore, the impact of the RecSys itself on users' decisions has not been appropriately isolated and quantitatively analyzed. To address these challenges, we propose a novel formulation of sequential recommendation, termed Causal Sequential Recommendation (CSRec). Instead of predicting the next item in the sequence, CSRec aims to predict the probability of a recommended item's acceptance within a sequential context and backtrack how current decisions are made. Critically, CSRec facilitates the isolation of various factors that affect users' final decisions, especially the influence of the recommender system itself, thereby opening new avenues for the design of recommender systems. CSRec can be seamlessly integrated into existing methodologies. Experimental evaluations on both synthetic and real-world datasets demonstrate that the proposed implementation significantly improves upon state-of-the-art baselines.

==> sections/Experiment_old.tex <==
\section{Experiment}
In this section, we incorporate CSRec into various baselines \cite{hidasi2016GRU4Rec, tang2018caser, SASRec2018, shin2024attentive, sun2019bert4rec} and compare the performance on both synthetic and real-world datasets. We demonstrate that CSRec universally outperforms the baselines and has a more robust performance. 

\subsection{Basic setup}
\label{sec:exp_setup}
\noindent\textbf{Datasets.} we evaluate \CSRec on two datasets: a real-world Spotify Sequential Music dataset\cite{brost2019music}, and a synthetic book dataset, GPT4-books where the generation details can be found in \Cref{app: exp-details}.

\MSSD was first introduced at the WSDM Cup 2019 Spotify Sequential Skip Prediction Challenge \cite{brost2019music}. The dataset contains approximately 160 million listening sessions, associated user actions, and 3.7 million tracks with acoustic features. The task is to predict whether a particular user will skip individual tracks encountered in a listening session. We use sessions sampled from personalized recommendations and user's own collections.

Given the limited access to interventional data, where the recommender system fully controls the exposure, we also created a synthetic dataset using GPT-4 as agents to mimic users' reactions to certain recommendations. We use the Amazon book dataset\cite{ni2019justifying} as a list of potential items to recommend. Then, we prepare a list of users, each with preferences across 10 genres. Detailed information and the prompt used can be found in \Cref{app: data-generation}. 


\noindent\textbf{Baselines and tasks.}
We compare CSRec with various sota baselines with different backbones: (1) RNN or CNN-based sequential models: GRU4Rec \cite{hidasi2016GRU4Rec} and Caser \cite{tang2018caser} and (2) transformer-based sequential recommender systems: SASRec \cite{SASRec2018}, BERT4Rec \cite{sun2019bert4rec}, FMLPRec \cite{Zhou2022FMLPRec}, and BSARec \cite{shin2024BSARec}. While CSRec can be incorporated into any sequential recommender systems, without loss of generality, we adapt the architecture of BSARec \cite{shin2024BSARec} with the new optimization loss to build our proposed model CSRec. We follow the basic setup as BSARec without additional hyper-parameter tuning.


We evaluate CSRec and the baselines models on both observational data where exposure is dominated by users and the interventional data where recsys controls the exposure.  On the observational data, we compare their performance in the task of forecasting the user's subsequent step from prior actions. While on the interventional data, we estimate the user's decision regarding a recommendation.

\noindent \textbf{Evaluation Metrics.}
\textit{Observational data: }
To have a comprehensive comparison between baseline models and CSRec, we measure the accuracy on both observational and interventional data. On observational data, we compare CSRec and SR baselines via widely used Top-k metrics, HR@k (Hit Rate) and NDCG@k (Normalized Discounted Cumulative Gain) where k is set to 5, 10, and 20 \cite{metrics_2020}.


% To verify the effectiveness of our model, we
% compare our method with well-known baselines in the task of (a) forecasting the user's subsequent step from prior actions on the observational data, and (b) estimation of user's decision regarding a recommended item on the interventional data. 
% Specifically, on observational data, we compare CSRec with baselines on how well the model predicts the next item given their prior spontaneous decisions. 
% Since our model is configured to take in both the recommended items and user's decisions, we can adapt our model to consider their reviews as surrogate decisions. 
% Specifically, on datasets that ranking/reviews are available, we use them as surrogate decisions and on datasets that these are unavailable, we treat decisions as positive for all items in the sequence.

% On interventional data, we examine how well models estimate user's decision when being recommended in interventional data. 
% For any conventional recommender systems, we feed in a users' spontaneous selected products, and convert to a binary decision from the ranking of the recommended item that the models computed.
% In other words, we apply an indicator function on the ranking such that the prediction is considered to be $1$ if the ranking is in the top-$\alpha$-percent.

% We include baselines with the following two categories, all designed to predict user's next move given their historical action sequences: (1) RNN or CNN-based sequential models: GRU4Rec \cite{hidasi2016GRU4Rec} and Caser \cite{tang2018caser} and (2) transformer-based sequential recommender systems: SASRec \cite{SASRec2018}, BERT4Rec \cite{sun2019bert4rec}, FMLPRec \cite{Zhou2022FMLPRec}, and BSARec \cite{shin2024BSARec}.

% \noindent\textbf{Model architecture.} We adapt the architecture of BSARec \cite{shin2024BSARec} with the new optimization loss to build our proposed model CSRec. To compute the constraint in the loss function \Cref{eq:loss fn 2}, we use BSARec on observational dataset as the pretrained model. We follow the basic setup as BSARec without additional hyperparameter tuning.


\textit{Interventional data: }
On interventional data, we compare the prediction of users' decisions through an adjusted hit rate (AHR). Moreover, we test the ability to predict users' decisions for the next $\beta$ time steps. For CSRec, the model outputs the predicted users' preference probability for the next $\beta$ recommended items. We then compare the resulting probability with the decisions $\in \{0,1\}$ via a binary cross entropy (BCE) loss and adjusted hit rate
\begin{equation}
    \text{AHR}_{\text{CSRec}} = \frac{1}{N\beta}\sum_N \sum_\beta \delta(d_t,\hat{d}_t), \quad \hat{d}_t = \chi_{\geq 0.8}(z_t)
\end{equation}
where $z_t$ is the model output, $\delta(a,b) = 1$ when $a = b$ and zero otherwise, and $\chi_A(x)$ is an indicator function such that it equals to 1 when $x \in A$ and zero otherwise.
For baseline models, we consider the users' decision to be $1$ whenever the predicted score for recommended items are in the top-20-percent $\mathcal{A}_{20}$. We then compute the binary cross entropy and adjusted hit rate.
\begin{equation}
    \text{AHR}_{\text{baselines}} = \frac{1}{N\beta}\sum_N \sum_\beta \delta(d_t,\hat{d}_t), \quad \hat{d}_t = \chi_{\mathcal{A}_{20}}(z_t)
\end{equation}



\subsection{Experimental results}

\begin{table}[h]
\vspace{-1em}
\caption{Compare with baselines with 3-step prediction ( $\beta = 3$)}
  \label{tab:scores}
  \begin{center}
  \scriptsize
  \begin{tabular}{p{1.cm}p{0.5cm}lccccccc}
    \toprule
    Dataset &  & Metric & GRU4Rec & Caser & SASRec & BERT4Rec & FMLPRec & BSARec & CSRec \\
    \midrule
    \multirow{8}{*}{GPT4-Books} & \multirow{6}{*}{$X_{\text{obs}}$} & $\uparrow$ HR@5  & 0.0477 & 0.0517 & 0.0529 & 0.0500 & 0.0474 & 0.0500 & \textbf{0.0807} \\
     &  & $\uparrow$ HR@10 & 0.0956 & 0.1014 & 0.1049 & 0.1023 & 0.1015 & 0.1000 & \textbf{0.1800} \\
     &  & $\uparrow$ HR@20 & 0.1991 & 0.2033 & 0.2039 & 0.1979 & 0.2042 & 0.2031 & \textbf{0.3155}\\
     &  & $\uparrow$ NDCG@5 & 0.0282 & 0.0302 & 0.0309  & 0.0295 & 0.0285 & 0.0294 & \textbf{0.0405} \\
     &  & $\uparrow$ NDCG@10 & 0.0435 & 0.0461 & 0.0475 & 0.0463 & 0.0458 & 0.0453 & \textbf{0.0721}\\
     &  & $\uparrow$NDCG@20 & 0.0694 & 0.0715 & 0.0722 & 0.0701 & 0.0715 & 0.0712 & \textbf{0.1061}\\
     \cmidrule{2-10}
    & \multirow{2}{*}{$X_{\text{intv}}$}& $\uparrow$ AHR & 0.2435 & 0.2434 & 0.2455 & 0.2430 & 0.2468 & 0.2423 & \textbf{0.8157}\\
     &  & BCE $\downarrow$ & 75.65 & 75.66 & 75.45 & 75.70 & 75.32 & 75.77 & \textbf{1.1366} \\
     % \midrule
     % \multirow{8}{*}{Book 0510} & HR@5 & 0.0957 & 0.2385 & 0.2411 & \textbf{0.2487} & 0.2207 & 0.2449 & 0.2207 \\
     % & HR@10 & 0.1952 & \textbf{0.4668} & 0.4464 & 0.4592 & 0.4311 & 0.4579 & 0.4554\\
     % & HR@20 & 0.3546 & 0.8151 & 0.7997 & 0.7985 & 0.7691 & 0.7959 & \textbf{0.8622}\\
     % & NDCG@5 & 0.0568 & 0.1491 & 0.1429 & 0.1540 & 0.1301 & \textbf{0.1568} & 0.1104\\
     % & NDCG@10 & 0.0887 & 0.2227 & 0.2086 & 0.2215 & 0.1974 & \textbf{0.2247} & 0.1858\\
     % & NDCG@20 & 0.1287 & \textbf{0.3112} & 0.2979 & 0.3073 & 0.2833 & 0.3103 & 0.2891\\
     % & AHR & 0.5697 & 0.6730 & 0.6709 & 0.6636 & 0.6653 & 0.6633 & \textbf{0.6802} \\
     % & BCE $\downarrow$ & 43.03 & 32.70 & 32.91 & 33.63 & 33.46 & 33.67 & \textbf{0.6683} \\
     \midrule
     \multirow{8}{*}{MSSD} & \multirow{6}{*}{$X_{\text{obs}}$} & $\uparrow$ HR@5 & 0.0148 & 0.0286 & 0.0429 & 0.0341 & 0.0745 & 0.1039 & \textbf{0.1505} \\
     & & $\uparrow$ HR@10 & 0.0312 & 0.0457 & 0.0981 & 0.0771 & 0.1031 & 0.2114 & \textbf{0.3041}\\
     & & $\uparrow$ HR@20 & 0.0773 & 0.0717 & 0.1227 & 0.0985 & 0.1592 & 0.2793 & \textbf{0.5889}\\
     & & $\uparrow$ NDCG@5 & 0.1045 & 0.0963 & 0.0845 & 0.0219 & 0.1487 & 0.1736 & \textbf{0.3719}\\
     & & $\uparrow$ NDCG@10 & 0.3112 & 0.1012 & 0.1082 & 0.0407 & 0.1952 & 0.1901 & \textbf{0.4007}\\
     & & $\uparrow$ NDCG@20 & 0.4410 & 0.0331 & 0.2110 & 0.7689 & 0.2747 & 0.2878 & \textbf{0.4372}\\
     \cmidrule{2-10}
     & \multirow{2}{*}{$X_{\text{intv}}$} & $\uparrow$ AHR & 0.1117 & 0.1461 & 0.1926 & 0.1468 & 0.1412 & 0.1692 & \textbf{0.6761} \\
     & & BCE $\downarrow$ & 2.4135 & 1.6079 &  5.2813 & 1.9130 & 2.7751 & 1.1498 &\textbf{0.0428} \\
  \bottomrule
\end{tabular}
\end{center}
\vspace{-1em}
\end{table}
% 

\noindent \textbf{Result analysis.}
As shown in \Cref{tab:scores} our method outperforms all baselines on all the metrics. Since baselines models are trained and optimized on observational data, they all have very similar performance on the interventional one. In comparison, CSRec is able to surpasses all benchmark models with a notably higher AHR and smaller BCE. Despite that our model is designed to accommodate interventional setting, it achieves better score than all baseline models by a significant margin via maintaining the underlying causal structures. 





==> sections/app4_tables.tex <==
\begin{table*}[h]
\caption{Results for CSRec integrated with baselines SASRec, BERT4Rec, FMLPRec and BSARec on GPT4-books using AHR@0.2 and AHR@0.5. CSRec + <model> represents the performance of CSRec integrated with baseline <model>.}
\vspace{-0.5em}
  \label{tab:improv}
  \begin{center}
  % \scriptsize
  \begin{tabular}{lcccccccc}
    \toprule
     Metric & SASRec & CSRec + SASRec & BERT4Rec & CSRec + BERT4Rec & FMLPRec & CSRec + FMLPRec & BSARec & CSRec + BSARec \\
    \midrule
    $\uparrow$ AHR@20 & 0.2438 & 0.3914 & 0.2430 & 0.3046 & 0.2435 & 0.932 & 0.2405 & 0.925\\
    $\uparrow$ AHR@50 & 0.4981 & 0.9176 & 0.5068 & 0.9153 & 0.5006 & 0.932 & 0.5037 & 0.932\\
     % BCE - 20 $\downarrow$ &75.623 & 60.86  & 75.953 &  & 75.647 & 6.773 & 75.697 & 7.51 \\
  \bottomrule
\end{tabular}
\end{center}
% \vspace{-1em}
\end{table*}
